Towards Ubiquitous Intelligent Hand Interaction

The development of ubiquitous computing and sensing devices has brought about novel interaction scenarios such as mixed reality and IoT (e.g., smart home), which pose new demands for the next generation of natural user interfaces (NUI). Human hand, benefit for the large degree-of-freedom, serves as a medium through which people interact with the external world in their daily lives, thus also being regarded as the main entry of NUI. Unfortunately, current hand tracking system is largely confined on first perspective vision-based solutions, which suffer from optical artifacts and are not practical in ubiquitous environments. In my thesis, I rethink this problem by analyzing the underlying logic in terms of sensor, behavior, and semantics, constituting a research framework for achieving ubiquitous intelligent hand interaction. Then I summarize my previous research topics and illustrated the future research directions based on my research framework.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> accessibility.tex <==
Figure 1. An example VR usage scenario enabled by ShadowTouch. (a) The user is sitting at a desk and browsing a photo album in VR environment. (b) With ShadowTouch, the user can turn the physical surface into a multi-touch interface, and perform a thumb-index multi-stroke gesture with aligned haptic feedback to make transformations of the photo.

Figure 2. The working principle of ShadowTouch. The light source is mounted on the root of the palm, with the hight of h_L. The fingertip is near the surface, with the hieght of h_F. 
D_H represents the projected distance between the light source and the fingertip on the surface, while d_S is the distance between the tip of the yielded shadow.

Figure 3. The hardware prototype of ShadowTouch. (a) The camera mounted on a Quest 2 HMD, with a down-facing angle of 45 degree. (b) A wearing example of the wristband. The light widget stretches to the root of the palm. (c) Specifications of the light widget (45mm length x 15mm height).

Figure 4. The algorithm pipeline of ShadowTouch. Given a series of video frames, the pipeline first extracts dynamic-size fingertip regions with MediaPipe. Then a pretrained MobileNet V3 model is applied to extract the features of the cropped images. Finally, the model runs a multi-layer perceptron (MLP) classifier to acquire the touch state prediction.

Figure 5. Data collection settings. (a) Apparatus and setup. (b) An example of camera capture (cropped to highlight the hand region). (c) The selected background textures other than the white background.

Figure 6. Examples of error cases: (a) The pinky finger is obstructed by other fingers. (b) Errors of MediaPipe fingertip recognition.

Figure 7. Application prototypes of ShadowTouch. (a) Home navigator. A screen is displayed in front of the user, with a cursor and three app icons. The user puts their hand on a horizontal virtual "trackpad".  (b) Photo album. A photo is displayed on the screen. The user can swipe or perform zooming gestures on the "trackpad". (c) Whiteboard. A whiteboard is displayed on the left of the trackpad. The user can draw on the canvas or select brushes on the brush panel. (d) Text Editor. A keyboard is displayed on the left of the trackpad. The user taps on a key to perform input.

Figure 8. NASA TLX Result, comparing between different interaction and techniques. Scores range from 1 to 7, with higher scores indicating lower demand / better performance / less effort and frustration.

Figure 9. System Usability Scale (SUS) Result across four different usage scenarios. 1 - strongly disagree, 5 - strongly agree.

Table 1. Accuracies, precisions, recalls, and F-1 scores of our evaluation in two training strategies and three window sizes. Numbers in the table are in percentage. A 5-frame window with the frame reloading strategy achieved an optimal performance of  99.1% 
 in accuracy and 96.8% in F-1 score across all fingers in recognizing finger touch state.

Table 2. Descriptions of atomic interactions in four applications and their categorization.

Table 3. The template scripts used by the experimenter to guide the user study tasks in four applications.


==> draft.tex <==

Introduction

精确指点、光标控制任务

现有的移动/可穿戴式光标控制设备xxx，例如指套xxx，有xxx问题

DualRing提出了支持指尖fingerpad的方案，但只是一个原型，1）对于光标映射的算法未充分研究，2）设计细节未充分地细化。我们希望优化DualRing上的touchpad应用。

本文的研究问题包括:


我们的贡献为:



Related Work


DR-PAD Design：

DR-PAD Algorithms：


Study 1: Algorithm Evaluation

Absolute

Relative


Study 2: Performance Evaluation

Fitts Law in 5 settings:

mouse, touchpad, DRPad (desktop), VR controller, DRPad (VR).

Results:

performance:

elapsed time for each phase: rest, touch, move.

touch point trajectory: smoothness, consistence, gesture speed

subjective perceptions.



Study 3: Usability Evaluation

在几个典型的application scenarios中评测（例如桌面、TV、AR/VR）
DR-Pad v.s. Mouse v.s. TouchPad v.s controller 

% 具体应用或任务，例如返回home、在列表中选择一个对象、浏览器中的浏览操作、离散菜单的导航等。

Missing related work

[Heat trace]
Daisuke Iwai and Kosuke Sato. 2006. Limpid desk: see-through access to disorderly desktop in projection-based mixed reality. In Proceedings of the ACM symposium on Virtual reality software and technology (VRST '06). Association for Computing Machinery, New York, NY, USA, 112–115. https://doi.org/10.1145/1180495.1180519
Eric Larson, Gabe Cohn, Sidhant Gupta, Xiaofeng Ren, Beverly Harrison, Dieter Fox, and Shwetak Patel. 2011. HeatWave: thermal imaging for surface user interaction. In Proceedings of the SIGCHI Conference on Human Factors in Computing Systems (CHI '11). Association for Computing Machinery, New York, NY, USA, 2565–2574. https://doi.org/10.1145/1978942.1979317
S. Brahmbhatt, C. Ham, C. C. Kemp and J. Hays, "ContactDB: Analyzing and Predicting Grasp Contact via Thermal Imaging," 2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), 2019, pp. 8701-8711, doi: 10.1109/CVPR.2019.00891.

[Fingernail color]
Naoki Sugita, Daisuke Iwai and Kosuke Sato, "Touch sensing by image analysis of fingernail," 2008 SICE Annual Conference, 2008, pp. 1520-1525, doi: 10.1109/SICE.2008.4654901.
Patrick Grady, Chengcheng Tang, Samarth Brahmbhatt, Christopher D. Twigg, Chengde Wan, James Hays, Charles C. Kemp. PressureVision: Estimating Hand Pressure from a Single RGB Image. ECCV 2022.

MirrorTrack - a vision based multi-touch system for glossy display surfaces. VIE 2008
SymmetriSense: Enabling Near-Surface Interactivity on Glossy Surfaces using a Single Commodity Smartphone. CHI 2016
Shadow reaching: a new perspective on interaction for large displays. UIST 2007 Shadow tracking on multi-touch tables. AVI 2008
A Camera Based Virtual Keyboard with Touch Detection by Shadow Analysis. Joseph Thomas 2013
A robust projector–camera interactive display system based on finger touch control by fusing finger and its shadow. JSID 2017
ShadowSense: Detecting Human Touch in a Social Robot Using Shadow Image Classification. IMWUT 2020
Detection of Finger Contact with Skin Based on Shadows and Texture Around Fingertips. HCII 2021


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> revision.tex <==
Practical Touch Tracking on Surfaces with Hybrid Depth-Infrared Sensing 

==> rw_backup.tex <==
\section{Related Work}

% McIntosh et al. 
% SensIR: Detecting Hand Gestures with a Wearable Bracelet using Infrared Transmission and Reflection
% \cite{10.1145/3126594.3126604}

% \cite{10.1145/3491102.3517440}
% ReflecTouch: Detecting Grasp Posture of Smartphone Using Corneal Reflection Images


% Sensible Shadow: Tactile Feedback from Your Own Shadow \cite{0.1145/2875194.2875199}

% HALUX: Projection-Based Interactive Skin for Digital Sports \cite{10.1145/2929464.2929479}

% \cite{10.1145/3242587.3242635}
% Self-Powered Gesture Recognition with Ambient Light

% \cite{10.1145/3191772}
% Gesture Recognition Using Ambient Light

% \cite{10.1145/2582051.2582090} Anywhere Surface Touch (most similar to our work) (xxx)

% \cite{10.1145/2992154.2996777} Touch Detection System for Various Surfaces Using Shadow of Finger



% https://www.youtube.com/watch?v=WZCDBZBY9lc

% 1.shadow (gestures) as input

% 2.free interface

% 3.?

% 1、Immersive Environment中的实体chumo交互（或者主动、被动触摸反馈）的好处、形式、代表技术/交互方式等
% Physical surface can improve user experience in virtual environment
\subsection{Physical-Aligned Touch Interaction in Immersive Environment}

% need more papers
Adopting physical settings or surfaces in the environment to provide haptic feedback in VR/AR has found interest in Mixed Reality communities. Offering passive haptic feedback with the help of physical entities in the environment has more advantages in reducing fatigue \cite{10.1145/3411764.3445302,10.1145/3472749.3474810}, improving the accuracy of hand gesture input \cite{10.1145/3411764.3445302} or sketch input\cite{10.1145/3025453.3025474,10.1145/3411764.3445302}, rich the set of interaction paradigms \cite{10.1145/2047196.2047255}, etc. For instance, Yang et al. \cite{10.1145/3332165.3347869} adopted the user's skin as a convenient surface for tactile touch-driven interactions to enable precise on-skin touch segmentation. Also using the human body for tactile feedback, Fang et al. \cite{10.1145/3472749.3474810} explored self-haptics where the user's right hand physically feels a keypad surface for interaction. OmniTouch \cite{10.1145/2047196.2047255} enabled the user to use their hands, arms, and legs as graphical, interactive surfaces as well as appropriate surfaces from the environment to expand the interactive area. For 3D sketch input tasks in VR/AR, touching a physical rigid surface for sketching has proved to improve the accuracy \cite{10.1145/3025453.3025474,10.1145/3173574.3173759,10.1145/3313831.3376628,10.1145/3173574.3173812,10.1145/3411764.3445302,10.1145/3550305}. Arora et al. \cite{10.1145/3025453.3025474} conducted a study that indicated drawing on a physical surface in VR performed better than projecting to virtual planes in the accuracy of the sketching. Jiang et al. \cite{10.1145/3411764.3445302} implemented VR physical gloves which enable one user's non-dominant hand as a canvas and the dominant hand as the painter to provide physical feedback in 3D sketching. 

In line with these works, we also adopted physical surfaces to provide tactile feedback in the  environment but ShadowTouch has more interactive capabilities for ubiquitous input in that it does not depend on any augmented surfaces or created overlays, any flat physical surface (rigid or soft) in the environment can be interactive in our system. 

% first, the interactive surface need not be instrumented. Secondly, this approach allows touch sensing on non-flat surfaces

% the interactive surface need not be instrumented
% % % 他们xxxx，我们只要满足一定光照条件的任意平整表面都可以提供物理反馈



% ----------------------------------------------------------------------

% Foremost, the system allows the wearer to use their hands, arms and legs as graphical, interactive surfaces. Users can also transiently appropriate surfaces from the environment to expand the interactive area (e.g., books, walls, tables).





% \cite{10.1145/3490149.3501320} demonstrated the 

% \cite{10.1145/3490149.3501320}Wristband wearable sensing for hand interaction: We demonstrate rich inferences about unaugmented everyday objects and hand object interactions by measuring minute skin surface deformations at the wrist using a sensing technique based on capacitance. 











% In line with 

% For instruments which provided positive physical feedback, for instance, 




% % 在虚拟环境里，有物理实体装置或表面具有很多方面的好处，例如，减少疲劳程度，提高用户操作的准确度，等等。许多研究都致力于在vr中引入可交互实体，分为主动交互（）和被动交互，主动交互的有xx，xx，xx





% \cite{10.1145/3332165.3347869}Actitouch:Contemporary AR/VR systems use in-air gestures or handheld controllers for interactivity. This overlooks the skin as a convenient surface for tactile, touch-driven interactions, which are generally more accurate and comfortable than free space interactions. In response, we developed ActiTouch, a new electrical method that enables precise on-skin touch segmentation by using the body as an RF waveguide. 



% \cite{10.1145/3025453.3025474}
% Physical Surface
% During our observational sessions, designers recommended projecting their strokes into desired virtual planes for greater accuracy. However, our experimental study indicates that, compared to accuracy achieved in traditional sketching, projecting to virtual planes in VR is 53\% worse, while drawing on a physical surface in VR is only 20\% worse. This is a strong motivation for devices combining existing drawing methods in VR. One potential approach is to hold a clipboard, or other rigid surface in the non-dominant hand to rest upon [33]. An alternative approach is dynamically configurable drawing surfaces actuated by robotic arms (Figure 13a). While the former potentially allows for higher mobility, the latter may be preferable in long design sessions where fatigue becomes a major factor. Such surfaces could potentially provide a more natural haptic feedback without limiting input range, unlike existing active haptic devices used to aid 3D sketching [27]. 

% \cite{10.1145/3472749.3474810} self-haptic advantages/ . In this work,
% we explore self-haptics (B), where through retargeting the user’s virtual hands, we can guide the physical hands together to create physical surfaces and objects for interaction – in this case, the user’s right hand physically feels a keypad surface. In this paper, we explore an alternative, highly mobile and controller-free approach
% to haptics, where VR applications utilize the user’s own body to
% provide physical feedback. (important!!!)

% \cite{10.1145/3411764.3445302}3d painter: lack of physical surface could lead to inaccuracy and fatigue

% \cite{10.1145/3490149.3501320}Wristband wearable sensing for hand interaction: We demonstrate rich inferences about unaugmented everyday objects and hand object interactions by measuring minute skin surface deformations at the wrist using a sensing technique based on capacitance. 



\subsection{Recognizing Touch on Unmodified Surface}
% Sensing touch accurately on unmodified everyday surfaces is an efficient way to improve the 

% is a fundamental task in HCI community. Touches on unmodified everyday surfaces 

% scratch input: \cite{10.1145/1449715.1449747}
Different sensing methods including IMU \cite{10.1007/978-3-319-58750-9_26,10.1145/3332165.3347947,10.1145/3432204,10.1145/3478114}, vibration sensing \cite{10.1145/3126594.3126619,10.1145/3397309,10.1145/1753326.1753394}, pressure sensing \cite{10.1145/3130978,10.1145/3430524.3442447,s21030859}, acoustic sensing \cite{10.1145/3338286.3340147,10.1145/1449715.1449747,paradiso2005tracking,YANG20131272} and optical sensing \cite{10.1145/1979742.1979715,10.1145/2047196.2047233,grady2022pressurevision,7223324,4384130} have been widely attempted to sense touches on everyday unmodified surfaces. 

IMU has a rich sensing capability to sense various hand activities but most related works did not focus on the touch state or achieving a satisfying accuracy of the whole process of a touch (from touch town to touch up). \cite{}. For example, AnywhereTouch \cite{10.1007/978-3-319-58750-9_26} proposed a finger-tracking method using nailed-mounted IMU on arbitrary surfaces. While some IMU sensing works focused on touch state, they were restricted to identifying individual finger touch events and can only recognize touching on a desk-like rigid surface. For example, Gu et al. \cite{10.1145/3332165.3347947,10.1145/3432204} implemented a finger ring with IMU to detect the touch state of individual fingers and further supports text entry on physical surfaces. TapID \cite{9417793,9419261} proposed a wrist-worn IMU device to sense precise touch events of individual finger and did not experiment on surfaces other than wooden office tables. Our work ShadowTouch has the capability to recognize precise multi-touch events without limitations of the contact surfaces.

Some finger-worn vibration or pressure sensing devices also attempted to sense touch: FingerPad \cite{10.1145/2501988.2502016} used a Hall sensor grid on the index fingernail and a magnet on the thumbnail to sense touch input. TypeAnywhere \cite{10.1145/3491102.3517686} used a wearable device that straps individually for fingers to decode typing sequences based only on finger-tap sequences without relying on tap locations. However, finger-worn devices \cite{9102253} limit fingers' flexibility for touching or daily activities so that affecting natural haptic feedback. ShadowTouch utilized a wrist-worn device that is not invasive to users' daily touching or hand activities.

Most of acoustic methods \cite{10.1145/3338286.3340147,10.1145/1449715.1449747,paradiso2005tracking,YANG20131272} mainly illustrated the capability of classifying hand gestures, general hand activities, and objects that actively emit acoustic signals \cite{10.1145/3397309}. AudioTouch \cite{10.1145/3338286.3340147} enabled a system that requires attaching two piezo-electric elements, acting as a surface mounted speaker and microphone, on the back of the hand to sense micro-gestures. However, ShadowTouch focused on recognizing the precise touch state on surfaces without any instrumentation.

Optical sensing which is ShadowTouch used has also been adopted to sense touch. For instance, Magic Finger \cite{10.1145/2380116.2380137} integrated an optical mouse sensor and an RGB camera into a device worn on the fingertip. 3DTouch \cite{7223324} coupled an optical laser sensor with a 9-DOF inertial measurement unit to support 3D interaction techniques, such as selection, translation, and rotation. Agarwal et al. \cite{4384130} detected touch locations and moments of contact with overhead stereo cameras, discussing how the noise from stereo depth causes erroneous proximity readings.  Optical sensing methods using depth cameras could help to recognize touch location, but the noisy depth data for reliable event detection is limited by camera framerates and applied filters \cite{9417793}. Our work ShadowTouch simply implements a low-cost camera without directly using the noise depth information, instead, we sensed the depth information by the shadow of the fingers which optimizes the effect for the touch state.

In summary, considering the scalability, accuracy, and non-invasive features mentioned above of sensing precise touch events on unmodified surfaces in daily life, we proposed to use optical methods without depth cameras to implement ShadowTouch.


% Gustafson et al. \cite{10.1145/2047196.2047233} also used a depth camera to provide more reliable detection and also scaled to mobile scenarios and on-body input.


% do not need any instrumentation for surfaces
%[tapid] we have not tuned or evaluated our method on its capability to identify multi-touch events—at this time, only individual fingers are detected, though with simultaneous bimanual input. A second as- sumption behind our current implementation is the use of a table or the user’s own body as a passive input surface We did not experi- mentally and quantitatively evaluate the detection accuracy of our current implementation on surfaces other than office tables made from coated wood. 


% [ready]\cite{10.1145/3397309}



% implemented a finger ring with IMU to detect the touch state . QwertyRing \cite{10.1145/3432204} utilized an IMU ring to supports text entry on physical surfaces. 

 

% \cite{10.1145/3130978}We present DigiTouch, a reconfigurable glove-based input device that enables thumb-to-finger touch interaction by sensing continuous touch position and pressure. Our novel sensing technique improves the reliability of continuous touch tracking and estimating pressure on resistive fabric interfaces

% % 我们用普通摄像头，通过影子感知到了深度信息

% works to use the low-cost camera without using the depth information to recognize the contour of 





% These camera-based approaches share the benefit of recognizing accurate touch locations, but all the struggle with noisy depth es- timates for reliable event detection and their constraints on input speed that is limited by camera framerates and applied filters. 



% optical:

% \cite{4384130}:Agarwal et al. detected touch locations and moments of contact with overhead stereo cameras [2], discussing how the noise from stereo depth causes erroneous proximity read- ings.





% \cite{10.1145/2380116.2380137}Magic Finger [59] integrated an optical mouse sensor and an RGB camera into
% a device worn on the fingertip

% \cite{7223324}Similarly, 3DTouch [36] coupled an optical laser sensor with a 9-DOF inertial
% measurement unit to support 3D interaction techniques, such as selection, translation and rotation. 3DTouch is
% closely related to ActualTouch.




% \cite{10.1145/3338286.3340147}AudioTouch:We present AudioTouch, a minimally invasive approach for sensing micro-gestures using active bio-acoustic sensing. It only requires attaching two piezo-electric elements, acting as a surface mounted speaker and microphone, on the back of the hand. It does not require any instrumentation on the palm or fingers; therefore, it does not encumber interactions with physical objects.




% However, most related works did not focus on touch detection or achieve a satisfying accuracy. 

% enabled touch input using magnetic tracking

% \cite{9417793}tapid,holz, This challenge is what we seek to complement with TapID, using wrist- worn inertial sensors that deliver the missing piece of information on rapid touch interaction: precise events and finger identification.


% \cite{10.1145/3332165.3347947}However, optical methods (i.e., with cameras on the headset) have difficulty in determining the touch contact accurately. We show that a finger ring with Inertial Measurement Unit (IMU) can substantially improve the accuracy of contact sensing from 84.74\% to 98.61\% (f1 score), with a low latency of 10 ms. We tested different ring wearing positions and tapping postures (e.g., with different fingers and parts).







% everyday passive objects


% inertial, vision, acoustic
% % 2、free-form hand-to-surface interaction, 传感原理（视觉、声学、惯性） - 传感能力（单指点击、多指点击、自由手势） - 交互功能

% ready, steady, and touch! \cite{}

% \cite{10.1145/2501988.2502016}fingerpad: FingerPad enables touch input using magnetic tracking, by adding a Hall sensor grid on the index fingernail, and a magnet on the thumbnail. magnet sensing

% \cite{10.1145/3432204}QwertyRing:In this paper, we present QwertyRing, a technique that supports text entry on physical surfaces using an IMU (Inertial Measurement Unit) ring. Users wear the ring on the middle phalanx of the index finger and type on any desk-like surface, as if there is a QWERTY keyboard on the surface. 

% \cite{10.1145/3130978}We present DigiTouch, a reconfigurable glove-based input device that enables thumb-to-finger touch interaction by sensing continuous touch position and pressure. Our novel sensing technique improves the reliability of continuous touch tracking and estimating pressure on resistive fabric interfaces

% \cite{10.1145/3338286.3340147}AudioTouch:We present AudioTouch, a minimally invasive approach for sensing micro-gestures using active bio-acoustic sensing. It only requires attaching two piezo-electric elements, acting as a surface mounted speaker and microphone, on the back of the hand. It does not require any instrumentation on the palm or fingers; therefore, it does not encumber interactions with physical objects.

% \cite{10.1007/978-3-319-58750-9_26}In this paper, we propose the AnywhereTouch, a finger tracking method using nailed-mounted inertial measurement unit (IMU) to allow a user to easily manipulate a virtual object on arbitrary surfaces. The AnywhereTouch activates recognizing process for touch input events when a user’s finger touches on an arbitrary surface. 

% \cite{10.1145/3126594.3126619}We developed a low cost prototype using piezo based vibration sensors attached to each finger. By combining the events from an input device with the information from the vibration sensors we demonstrate how to achieve low latency and robust finger identification.


% \cite{10.1145/3332165.3347947}However, optical methods (i.e., with cameras on the headset) have difficulty in determining the touch contact accurately. We show that a finger ring with Inertial Measurement Unit (IMU) can substantially improve the accuracy of contact sensing from 84.74\% to 98.61\% (f1 score), with a low latency of 10 ms. We tested different ring wearing positions and tapping postures (e.g., with different fingers and parts).

% \cite{10.1145/3491102.3517686}. Using a wearable device that can detect finger taps, users can leverage their touchtyping skills from physical keyboards to perform text entry on any
% surface. TypeAnywhere decodes typing sequences based only on finger-tap sequences without relying on tap locations.

% \cite{4384130}:Agarwal et al. detected touch locations and moments of contact with overhead stereo cameras [2], discussing how the noise from stereo depth causes erroneous proximity read- ings.

% \cite{9417793}tapid,holz, This challenge is what we seek to complement with TapID, using wrist- worn inertial sensors that deliver the missing piece of information on rapid touch interaction: precise events and finger identification.

% \cite{10.1145/3397309}A finger held in the air exhibits microvibrations, which are reduced when it touches a static object. When a finger moves along a surface, the friction between them produces vibrations, which can not be produced with a free-moving finger in the air. With an inertial measurement unit (IMU) capturing such motion characteristics, we demonstrate the feasibility to detect contact between the finger and static objects. We call our technique ActualTouch. 



% optical:
% \cite{10.1145/2380116.2380137}Magic Finger [59] integrated an optical mouse sensor and an RGB camera into
% a device worn on the fingertip

% \cite{7223324}Similarly, 3DTouch [36] coupled an optical laser sensor with a 9-DOF inertial
% measurement unit to support 3D interaction techniques, such as selection, translation and rotation. 3DTouch is
% closely related to ActualTouch.

% FingerPad: private and subtle interaction using fingertips

% \cite{10.1145/1753326.1753394}skininput[16]:Assisted by other sensing techniques, such as acoustic sensors [16] or an IR laser [32], they can easily turn a surface into an interactive interface. In particular, we resolve the location of finger taps on the arm and hand by analyzing mechanical vibrations that propagate through the body

% \cite{10.1145/1979742.1979715}[32]

% \cite{10.1145/2992154.2992173}In this paper we present DIRECT, a novel touch-tracking algorithm that merges depth and infrared imagery captured by a commodity sensor. This yields significantly better touch tracking than from depth data alone, as well as any prior system.



% imu/tremal: cannot broad to any surface
% \cite{}





% depth data is not good enough for sensing touch contactness! so we proposed the utilize the shadow of the finger touching a surface  to optimize the effect for the touch state

% 我们只需要一个附着在手上的光源，并且利用在vr头盔上现有的camera，就可以实现精准的touch state检测。

\subsection{Enhancing Vision-based Hand Gesture Recognition with Auxiliary Optical Instruments}
% 3、基于光学/物理结构/xxx的视觉传感增强(比如像handsee这种，核心是去构造一些硬件设定使得一个视觉检测任务从不可识别/识别不好到可识别/识别好，这类型的工作，title可以再想想) 
%这个title是不是好一点
%Enhancing Vision-based Hand Gesture Recognition with Auxiliary Optical Instruments

% \cite{10.1145/2992154.2996777}Touch Detection System for Various Surfaces Using Shadow of Finger

% \cite{10.1145/2582051.2582090} Anywhere Surface Touch (most similar to our work) (xxx)



Auxiliary optical instruments to improve the capability of vision-based hand recognition have been extensively researched. 

Mirrors are the most widely-used choice for enhancing optical channels in that they can provide  multiple views for the above surface which potentially enables stereo gesture recognition \cite{10.1145/3411764.3445583,9176728,10.1145/2501988.2502049,10.1145/2999508.2999522,10.1145/3290605.3300935}. Matulic et al. \cite{10.1145/3411764.3445583} proposed a mounting mirror above the phone screen so that the front-facing camera captures the thumbs on or near the screen. Lim et al. \cite{9176728} utilized plane mirrors to create multiple views of the hand to reduce the issues of occlusion, and the error in measuring the flexion angle of finger joints. Yang et al. \cite{10.1145/2501988.2502049} attached an omni-directional mirror to the front camera to enable peripheral vision around the device. Yu et al. \cite{10.1145/3290605.3300935} used a prism mirror placed on the front camera to create a stereo vision system that generates a depth image of the hand for tracking finger location and movement. 

Other optical instruments such as photovoltaic mode were used by Li et al. \cite{10.1145/3191772} to sense touch and near-range finger gestures. Chen et al. \cite{10.1145/2642918.2647392} researched the design space of the mid-air hand gestures using a depth camera mounted on the phone. ReflecTouch \cite{10.1145/3491102.3517440} detected the grasping posture of smartphones by the reflection images of corneal. 


However, most works above focused on exploring more interactive space for hand gestures, for example, the 3D hand gestures above a surface \cite{10.1145/3290605.3300935,10.1145/2642918.2647392,10.1145/3191772,10.1145/3332165.3347904,10.1145/2501988.2502049,10.1145/3379337.3415818,10.1145/1294211.1294259,10.1145/3384657.3384797}. Our work is different from their attempts that we focused more on distinguishing the subtle touch state (contact and non-contact) of fingers on physical surfaces, as well as more accurate gesture interaction such as the switch between transient gestures (from single finger click to multiple finger click, from single finger click to multiple finger drag, etc). 

Detection the fingers' projection or reflection of light sources has also been explored by many research \cite{10.1145/2582051.2582090,10.1145/2992154.2996777}. Niikura et al. \cite{10.1145/2992154.2996777} utilized an infrared (IR) camera and two IR lights to detect the shadows of a finger, but their system needed augmented surfaces to put IR cameras and lights. Another research of Niikura's \cite{10.1145/2582051.2582090} is the most similar to ShadowTouch which also utilized wrist-worn LEDs and a camera to recognize the interacting and in which direction the fingers are moving. However, their system required a camera worn between the wrist and the surface which leads the hand and the forearm hovering in the air to cause a lot of fatigue. Furthermore, though their sensing system recognized contact by fusing visual and sound, the precise contact state cannot be distinguished due to the finger regions are connected in an obtained image. ShadowTouch also utilized the finger's projection while our system combined the features of the fingers' shadow and the fingers which enables the precise contact state detection and our form fact is more non-invasive to users for we do not have much sensing elements worn by the wrist.

% The system recognizes which fingers are interacting and in which direction the fingers are moving.
% Additionally, to recognize the contact con- ditions, we installed a contact microphone next to the camera to obtain sounds from the surface. The system recognizes the contact by fusing visual and sound information.

% their system recognized the 

% contact by fusing visual and sound cannot distinguish the performing fingers 

% The fingers which were next to one performing gesture
% were also misrecognized as performing gesture

% The second misrecognition is due to the subjects’ mistake, or the finger regions are connected in an obtained image. During performing the gesture, if the fingers near the base of the finger are close, the finger regions in the obtained image may be connected, and this causes the the failure of finger tracking.

% Our work is different from their attempts that we focused more on distinguishing the subtle touch state (contact and non-contact) of fingers on physical surfaces, as well as more accurate gesture interaction such as the switch between transient gestures (from single finger click to multiple finger click, from single finger click to multiple finger drag, etc). 

% 写的咋样 能用不
% 找的工作还行，现在基本上是在列工作，差一些逻辑上的组织

% (need more insights, e.g., why these instruments are needed, how can they enhance visual hand gesture recognition, what categories, more underlying logic and motivation) 




% detected touch gestures through a mirror's reflection on the back of the phone.


% Back-Mirror consists of two main parts: a smartphone accessory with a mirror that can reflect the back surface to the rear-facing camera of the phone, and a computer-vision algorithm for gesture recognition based on the visual pattern on the back surface. 

% 通过增强光学信道来提高从视觉方向识别手势交互的能力已经被广泛的研究。xx xx xx。然而，这些工作大多数集中于拓展了手势交互的交互空间，例如xx，xx，xx引入的的3D手势交互等，而我们更关注手指在接触和非接触物理表面的细微差别，以及瞬态手势的切换等更精准的手势交互识别。




% \cite{10.1145/3379337.3415818} We present DeepFisheye, a practical NMFT solution for mobile devices, that utilizes a fisheye camera attached at the bottom of a touchscreen. 

% \cite{9176728}We proposed a multi-view setup using a readily avaiable color camera from a single mobile phone, and plane mirrors to create multiple views of the hand. reduce the issues of occlusion, reduce the error in measuring the flexion angle of finger joints.

% \cite{10.1145/3411764.3445583} We propose mounting a mirror above the phone screen such that the front-facing camera captures the thumbs on or near the screen. This enables the creation of semi-transparent overlays of thumb shadows and inference of fingertip hover points with deep learning, which help the user aim for targets on the phone. 3d gestures

% \cite{10.1145/3491102.3517440}
% ReflecTouch: Detecting Grasp Posture of Smartphone Using Corneal Reflection Images

% \cite{10.1145/3290605.3300638}We present Magnetips, a simple, mobile solution for around-device tracking and mid-air haptic feedback. Magnetips combines magnetic tracking and electromagnetic feedback that works regardless of visual occlusion, through most common materials, and at a size that allows for integration with mobile devices

% \cite{10.1145/2642918.2647392}use a depth camera mounted on the phone to track hands and fingers in mid-air.

%  \cite{10.1145/3332165.3347904}Based on design considerations for interaction, mobility, and object appearance and physics, we implemented a prototype for portable 3D hand tracking using a smartphone, a Leap Motion controller, and a computation unit. 
 
%  \cite{10.1145/2501988.2502049}Yang et al. attach an omni-directional mirror to the front camera to enable peripheral vision around the device. We present Surround-See, a self-contained smartphone equipped with an omni-directional camera that enables peripheral vision around the device to augment daily mobile tasks.
 
%  \cite{10.1145/1294211.1294259}In this paper, we present LucidTouch, a mobile device that addresses this limitation by allowing the user to control the application by touching the back of the device. LucidTouch supports back-of-device multitouch input with a see- through effect for the fingers using a camera mounted behind the device to capture the hands 
 
%  \cite{10.1145/2999508.2999522}We present Back-Mirror, a low-cost camera-based approach for widening the interaction space on the back surface of a smartphone by using mirror reflection. 
